Latent Space Model for Road Networks to Predict Time-Varying Traffic

Real-time traffic prediction from high-fidelity spatiotemporal traffic sensor datasets is an important problem for intelligent transportation systems and sustainability. However, it is challenging due to the complex topological dependencies and high dynamics associated with changing road conditions. In this paper, we propose a Latent Space Model for Road Networks (LSM-RN) to address these challenges. In particular, given a series of road network snapshots, we learn the attributes of vertices in latent spaces which capture both topological and temporal properties. As these latent attributes are time-dependent, they can estimate how traffic patterns form and evolve. In addition, we present an incremental online algorithm which sequentially and adaptively learn the latent attributes from the temporal graph changes. Our framework enables real-time traffic prediction by 1) exploiting real-time sensor readings to adjust/update the existing latent spaces, and 2) training as data arrives and making predictions on-the-fly with given data. By conducting extensive experiments with a large volume of real-world traffic sensor data, we demonstrate the utility superiority of our framework for real-time traffic prediction on large road networks over competitors as well as a baseline graph-based LSM.

==> tex/data.tex <==
% data description
%We consider the loop detectors on the Los Angeles road network. There are totally 9300 sensors located on the highways and arterial streets of Los Angeles County (covering 5400 miles cumulatively). %The sampling rate of the sensor data is 1 reading/sensor/min. We average the readings over five consecutive time intervals. Therefore, 
%Each loop detector provides a traffic speed reading $v$ (e.g., miles/hour)  every 5 minutes from 6am to 9pm. Therefore, each sensor provides 180 distinct measurements per day.
%
%We formally define our problem from the sensor's perspective: 
%
%\begin{problem}
%Missing value prediction:  given a period of $T$ (e.g, one month), our task is to complete the missing value of  the sensor readings during the period of $T$.
%\end{problem}
%
%We could also formulate our problem in terms of building a spatial temporal network model:
%
%\begin{definition}
%Spatial temporal network:  a time-dependent graph is defined as $G(V, E, W)$: where $V$ is a set of nodes, $E$ is a set of edges. For every edge $(v_i, v_j) \in E$, there is a function $c_{i,j}(t)$, where $t$ is the time variable in time domain $W$. An edge cost function $c_{i,j}(t)$ specifies the travel cost from $v_i$ to $v_j$ starting at time $t$.
%\end{definition}
%
%\begin{problem}
%Given a road network $G=(V,E)$, the whole set of sensors with their readings over a time period of $T$ and the time granularity (e.g, weekly), our goal is to build a spatial temporal network $G(V, E, W)$ over the network $G$.
%\end{problem}

We want to predict the traffic condition of a road network at time $t+1$ given a sequence of its recent snapshots from time 1 to $t$. The road network is denoted as a directed graph $G=(V, E)$, where $V$ and $E\in V \times V$ is a vertex set and an edge set, respectively. A vertex $v_i\in V$ models a road intersection or an end of road. An edge $e_k = (v_i, v_j)$ models a directed road segment, which associates with an edge cost (i.e., travel time).

The road network snapshots are built from the readings of the loop detectors. 
9300 sensors are located on the highways and arterial streets of Los Angeles County (covering 5400 miles cumulatively).  %The sampling rate of the sensor data is 1 reading/sensor/min. We average the readings over five consecutive time intervals. Therefore, 
Each loop detector (sensor) provides a traffic speed reading (e.g., miles/hour)  every 5 minutes from 6am to 9pm, %Therefore, each sensor provides 180 distinct measurements per day. 
and is mapped to a specific edge in the underlying road network. Note that, typically sensors cannot span all the edges  of the road network because of its high costs. In our case, most of the highway edges are covered with sensors, whereas only a small amount of arterial edges (secondly streets) are covered with sensors.

We consider temporal dynamic link costs. Let $G_t =(V, E, W_t)$ be a road network snapshot recorded at time $t$, where $W_t$ represents the adjacency edge weights. We define our problem as follows:

\begin{problem}
    Given a sequence of network snapshots $(G_0, G_1, \cdots, G_t)$, we aim to predict the road network $G_{t+1}$.
\end{problem}

We divide one day into fine-grained slots (i.e., 5 minutes), therefore, the time interval between $G_i$ and $G_{i+1}$ is 5 minutes. In addition to the recent network snapshots $(G_0, G_1, \cdots, G_t)$, the input could also include the historical snapshots (e.g, yesterday's road network, averaged Monday road network). 

Potential challenges are listed as follows:

\begin{itemize}
\item{Data sparsity}: predict the travel time of edges without any sensors.

\item{Real-time prediction on directed weighted graph.} 

\item{Large scale:} the graph contains more than 100K nodes and 200K edges.

\item{Historical v.s. real time traffic:} How to effectively leverage the most relevant historical pattern?
\end{itemize}

==> tex/exp.tex <==
% experiment 
%\subsection{Experiment Design}
We conduct a set of experiments to verify our proposed methods.
\subsection{Datasets}
We select a sub highway network of LA which contains 5720 nodes and 5824 edges. We map our sensor dataset into the edge of 
our sub LA network. We use one week of April, 2015 (04/06 to 04/10) dataset of our experiments.

\subsection{Baseline method}
For the task of edge completion, we compare with one baseline method, which only uses the spatial topology for edge completion without considering the temporal factors.\dingedit{Tensor methods might also be used here!}

For static prediction of $G_{t+1}$, we compare with two methods: 1) use the previous Snapshot $G_t$ as the prediction of 
$G_{t+1}$, 2) for each edge, we train an ARIMA model and use it for prediction. \dingedit{other time series analysis method (e.g., HMM) could also be used here!}

For online prediction, our method ONMF is a conditional update method. To show the advantage of instant feedback, we compare our method with three baselines: 1) prediction without using any feedback, i.e., the latent space are always evolved as $U_t = U_{t-1}*A$ 2) always use the previous snapshot as the prediction, 3) recompute the latent space from scratch for the observed single snapshot.

\subsection{Configurations and Measures}
We vary two parameters, T and Span. T means the number of snapshots we are using per prediction. Span means the time range between two continuous snapshots.

We select two time ranges for our completion and prediction task, i.e., rush hour (5pm-6pm or 7am-8am) and non-rush hour (2pm-3pm or 8pm-9pm). \dingedit{decide a time range for prediction per day.}

We also conduct an experiment study on the event of XXXXXX.

We use mean absolute percent error (MAPE) and root mean square error (RMSE) to measure the accuracy.

\begin{equation*}
\begin{aligned}
MAPE = (\frac{1}{N}\sum_{i=1}^{N}\frac{|y_i-\hat{y_i}|}{y_i})\\
RMSE = \sqrt{\frac{1}{N}\sum_{i=1}^{N}(y_i-\hat{y_i})^2}
\end{aligned}
\end{equation*}



\dingedit{Notice how the transition matrix varies for different time ranges(i.e., rush, non-rush, event).}

\subsection{Edge completion evaluation}
The first set of experiments test how the completion accuracy  varies for rush hour and non rush-hour. In
this experiment we fix T=10, span=1.

The second set of experiments test the effect of T and span for both rush hour and non rush hour scenario.
We fix $T=\{4\}$, while span varies from $1, 2, 3, 4, 5, 6$. We fix $span=\{1\}$, when T varies from $3,5,7,9,10$.

Expected results for edge completion:

\begin{myans}
	Our method should perform much better than the topology approach when Span is small. The improvement becomes marginally when Span increases. In terms of T, the accuracy should increase or at least stay stable when T increases.
\end{myans}

\subsection{Static prediction evaluation}

The first set of experiments test how the prediction accuracy  varies for rush hour and non rush-hour. In
this experiment we fix T=6, span=1. For each rush hour range, we select 10 prediction points.

The second set of experiments test the effect of T and span for both rush hour and non rush hour scenario.
We fix $T=\{4\}$, while span varies from $1, 2, 3, 4, 5, 6$. We fix $span=\{1\}$, when T varies from $3,5,7,9,10$.

Expected results for static prediction:

\begin{myans}
	NMF improves when T increases, the improvement decreases when span increases. NMF should perform better than the previous snapshot and the ARIMA model. 
	\dingedit{Decide whether to predict Random edges or ALL edges}
\end{myans}

\subsection{Online prediction evaluation}
Expected results for online prediction:

\begin{myans}
	Our method should be much better than the methods without considering the instant feedback.
	\dingedit{Check the performance why ONMF is better than Recompute and Topology completion.}
\end{myans}

\subsection{TO-DO lists}
\begin{itemize}
	\item For the baseline algorithm: how to optimize the Armijo rule for block coordinate descent method. How to decide the latent number.
	\item Improve the prediction accuracy
	\item improve the efficiency of off-line and on-line NMF algorithm.
\end{itemize}

%\subsection{Small Dataset Description}
%As an exploratory study, we conduct a small scale experiment. We use two datasets for our testing purpose: namely $dense$ and $sparse$ datasets. 
%
%With $dense$,  we choose 115 sensors in the I-405 highway segment of LA with both north and south directions. We pick the sensor readings of one whole month at April, 2014.  Each sensor has a reading about the travel speed (i.e. miles/hour) in a 15 minutes interval from 6am to 9pm per day.
%
%With $sparse$, we randomly choose 100 sensors from 4 different highways ( I-405,  I-110,  I-605 and  I-710) with north and south directions. We also pick the sensor readings of one whole month at April, 2014. The distribution of sensors in $dense$ and $sparse$ are shown in Figure~\ref{} (To be added shortly).
%
%\subsection{Configurations and Measures}
%For each dataset, we randomly choose $5\%$ sensors as unobserved, and then predict their values.  We compare our prediction value with the real sensor readings and calculate the RMSD per dataset. We repeat this procedure 10 times and report the average of the RMSD.
%
%\subsection{Baseline}
% Our task is to predict the unobserved sensor values. For one unobserved sensor, the baseline algorithm uses the readings of its nearest neighbor as its prediction values. If the reading of the nearest neighbor sensor is missing, we use the reading of its second (or the third) nearest neighbor sensor. We compare our approach with the tensor approach. 
%%\dingedit{Simple description of the tensor approach?}
%%\ryedit{Description of the downsampled dataset}
%
%\subsection{Preliminary Result}
%Experiment results for baseline algorithm are shown in Table~\ref{tbl::rmsd}. The RMSD values of each round are shown in Table~\ref{tbl::rmsd-dense} and~\ref{tbl::rmsd-sparse}. Basically, baseline algorithm performs better on $dense$ than on $sparse$. The reason is that on $sparse$, for one sensor we want to predict, its nearby sensors are not necessarily located at the same highway segment, and they might not be a good choice for prediction.
%
%\begin{table*}[!ht]
%  \caption{Average RMSD value}
%  \centering
%  \begin{tabular}{| l | l | l |}
%    \hline
%       dataset & $dense$ & $sparse$  \\ \hline
% RMSD &23.387 & 30.933 \\ \hline
%  \end{tabular}
%  \label{tbl::rmsd}
%\end{table*}
%
%
%\begin{table*}[!ht]
%  \caption{RMSD value of each round for $Sparse$}
%  \centering
%  \begin{tabular}{| l | l | l | l | l | l | l | l | l | l | l |}
%    \hline
%       round & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10   \\ \hline
% RMSD &36.754&19.488&16.629&16.233&37.209&9.682&37.066&16.303&22.708&21.801\\ \hline
%  \end{tabular}
%  \label{tbl::rmsd-dense}
%\end{table*}
%
%
%\begin{table*}[!ht]
%  \caption{RMSD value of each round for $Sparse$}
%  \centering
%  \begin{tabular}{| l | l | l | l | l | l | l | l | l | l | l |}
%    \hline
%       round & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10   \\ \hline
% RMSD &35.441&47.146&15.475&16.467&28.438&46.058&35.875&35.652&26.908&21.867\\ \hline
%  \end{tabular}
%  \label{tbl::rmsd-sparse}
%\end{table*}






==> tex/intro.tex <==
% introduction
Many urban freeways are equipped with induction loop detectors. Three type of real time information are accessible from those detectors \cite{kwon2000modeling}: the number of vehicles passing the location during a given time interval (flow rate), the fraction of time that vehicles are over the detector (occupancy), and the vehicle velocities averaged over the time interval. The aggregated velocity is an important indicator of the traffic situation and is the direct estimator for travel time.

\begin{itemize}
    \item a unified framework for both data completion and prediction.
    \item (1) overcome sparse challenges via utilizing spatial topology, efficient global and incremental algorithms scale to large dataset. 
    (2) learn time-dependent latent space and transition matrix which captures the temporal trends. (3) require much less training data compared with traditional methods.
    \item incremental update, real-time incorporate the feedbacks.
    \item extensive experiments compared with many state-of-the-art methods!!!!!
\end{itemize}

==> tex/method.tex <==
%method
\subsection{Framework}
Describe the basic framework and the streaming framework.

\begin{figure}[!h]
    \centering
    \includegraphics[width=70mm]{fig/overall-framework}
    \vspace{-3mm}\caption{Overall Framework} \vspace{-5mm} \label{fig::framework}
\end{figure} 

\begin{figure}
    \centering
    \includegraphics[width=70mm]{fig/latentspace}
    \vspace{-3mm}\caption{Latent space learning} \vspace{-5mm} \label{fig::latent}
\end{figure}

\subsection{Data Completion Via Road Network Topology}
Because of the sparsity of our matrix, we utilize the topology of road network
to complete the edges without any readings. Meanwhile, we calculate a confidence
level for each completed edge, which represents how accurate this completion could be.

\subsubsection{Completion via Grid indexes}

\subsubsection{Edge Completion confidence computation}
\subsection{Basic Model description}
We consider how to learn two latent matrices from the current graph $G$.
We use a matrix $U \in R_{+}^{n\times k}$ to denote the attribute of the $n$ vertices
in $V$, a matrix $B \in R_{+}^{k \times k}$ to denote the attribute interaction matrix.
The product form $UBU^T$ represents the travel speed matrix between two vertices of the
graph, we want to use it to approximate the adjacency matrix $G$, as well as learn the 
speed for those unknown edges. 

The matrix $U$ represents the node attributes. For example, highway/arterial way,
business/residential area. For each entry $u_{ij}$ in $U$, we interpret it as the probability 
that vertex $i$ has the attribute $j$. 	We first assume that $0 \leq U \leq 1$.
% ToDo:
% how should we bound our matrix entry u??? 

The matrix $B$ represents the relationship between two attributes, i.e., the travel pattern from
one attribute to another attribute.

Because of the sparsity of matrix, we only consider the loss defined on the edges with $e_{ij} > 0$.
Define $I$ as the set of indices of all the non-zero entries in $G$, thus the objective function is defined as follows:

\begin{equation}
\arg\min_{U,B}J=\sum_{(i,j) \in I}(G(i,j) - U_iBU_j^T)_F^2
\end{equation}
  
We could also add a graph Laplacian constraint $L$ which captures the similarity between different nodes. Therefore, assume we have an indication matrix $Y$, the objective could be expressed as follows;  

\begin{equation}
J=||Y\odot (G-UBU^T)||_F^2 + \lambda Tr(U^TLU)
\end{equation}

Three algorithms are discussed to solve the above optimization problem.  
\subsubsection{Multiplicative Update (MU)}  

Take the derivative in respect of $U$ and $B$, we have the following:
\begin{equation}\label{eqn::uderi}
    \frac{\partial J}{\partial U}=-2(Y\odot G)(UB^T+UB) + 2(Y\odot UBU^T)(UB^T+UB)
\end{equation}


\begin{equation}\label{eqn::bderi}
    \frac{\partial J}{\partial B}=-2U^T(Y\odot G)U + 2U^T(Y\odot UBU^T)U
\end{equation}

The update rules is listed as follows:

\begin{equation}\label{eqn::mu-u}
    U_{ij}\leftarrow U_{ij} \Big(\frac{[(Y\odot G)(UB^T+UB)]_{ij}}{[(Y\odot UBU^T)(UB^T+UB)]_{ij}}\Big)^\frac{1}{4}\\
\end{equation}

\begin{equation}\label{eqn::mu-b}
    \begin{aligned}
        B_{ij}\leftarrow B_{ij} \Big(\frac{[U^T(Y\odot G) U]_{ij}}{[U^T(Y\odot (UBU^T))U]_{ij}}\Big)^\frac{1}{2}
    \end{aligned}
\end{equation}

\dingedit{check the value of $\frac{1}{2}$ for the updateing of $B$.}

The algorithm of MU is listed as follows:

\begin{algorithm}\small\caption{MU}
    \textbf{Input:} graph matrix $G$.\\
    \textbf{Output:}  $U$ and $B$. \\
    \vspace{-2mm}
    \label{alg::mu}
    \begin{algorithmic}[1]
        \STATE{Initilize U and B}
        \WHILE{Not Convergent}
            \STATE{update U with equation~\ref{eqn::mu-u}}
            \STATE{update B with equation~\ref{eqn::mu-b}}
        \ENDWHILE
    \end{algorithmic}
\end{algorithm}

\subsubsection{Block coordinate gradient descent (BCGD) method}
We update each row of the matrix $U$.
Specifically, 

\begin{equation}
\begin{aligned}
\Delta{J(u_i)} =
% &-2(\sum_{(i,j) \in I}(G(i,j)-U_iBU^T_j)(BU^T_j)^T + \\
% &\sum_{(j,i) \in I}(G(j,i)-U_jBU^T_i)(U^T_jB)^T)\\
 -2\sum_{j \in In(i)}(G(i,j)-u_iBu^T_j)u_jB^T\\
-2\sum_{j \in Out(i)}(G(j,i)-u_jBu^T_i)u_jB
\end{aligned}
\end{equation}

Therefore, we update $z^{r+1}(u)$ at iteration $r+1$ with the following rule:
\begin{equation}\label{eqn::bcgd-u}
u^{r+1}_i = \max(u^{r}_i - \alpha \Delta{J(u^{r}_i)}, 0)
\end{equation}

We could update $B$ with the same rule of MU. Alternatively, we could update with the
following rule from Equation~\ref{eqn::bderi}:

\begin{equation}\label{eqn::bcgd-b}
    B^{r+1} = \max(B^{r} - \alpha \frac{\partial J}{\partial B}, 0)
\end{equation}

\begin{algorithm}\small\caption{BCGD}
    \textbf{Input:} graph matrix $G$.\\
    \textbf{Output:}  $U$ and $B$. \\
    \vspace{-2mm}
    \label{alg::bcgd}
    \begin{algorithmic}[1]
        \STATE{Initilize U and B}
        \WHILE{Not Convergent}
            \FOR{each $i \in G$}
                \STATE{update $u_i$ with equation~\ref{eqn::bcgd-u}}
            \ENDFOR
        \STATE{update B with equation~\ref{eqn::bcgd-b}}
        \ENDWHILE
    \end{algorithmic}
\end{algorithm}

\subsubsection{Coordinate gradient descent method} 
We update each entry of the matrix $U$, and then $B$ separately.
The baseline algorithm could be referred to~\cite{zhang2012overlapping}, which could
be improved with the idea of~\cite{hsieh2011fast}. The idea is to selectively choose
an important entry of the matrix $U$, then solve a quadric function each time.

\subsubsection{Semi-nonnegative for the matrix $B$} 
The matrix $B$ might be allowed with negative number.

In this case, we might have an alternative way of updating $B$, i.e., a closed form solution:

\begin{equation}\label{eqn::semi-b}
B=(U^TU)^{-1}U^TGU(U^TU)^{-1}
\end{equation}
\dingedit{The above closed form solution is wrong because $Y$ has not been considered.}

For the MU algorithm, because B might contain negative value, the update rule of $U$ is modified as follows:

\begin{small}
\begin{equation}\label{eqn::semi-mu-u}
U_{ij}\leftarrow U_{ij} \Big(\frac{[\big((Y\odot G)(UB^T+UB)\big)^{+} + \big((Y\odot UBU^T)(UB^T+UB)\big)^{-}]_{ij}}
{[\big((Y\odot G)(UB^T+UB)\big)^{-} + \big((Y\odot UBU^T)(UB^T+UB)\big)^{+}]_{ij}}\Big)^\frac{1}{4}\\
\end{equation}
\end{small}
where we use $(\cdot)^+$ and $(\cdot)^-$ to denote the positive and negative parts of a matrix, 
$A^{+}=(|A|+A)/2$,$A^{-}=(|A|-A)/2$.


\begin{algorithm}\small\caption{Semi-MU}
    \textbf{Input:} graph matrix $G$.\\
    \textbf{Output:}  $U$ and $B$. \\
    \vspace{-2mm}
    \label{alg::semi-mu}
    \begin{algorithmic}[1]
        \STATE{Initilize U and B}
        \WHILE{Not Convergent}
            \STATE{update B with equation~\ref{eqn::semi-b}}
            \STATE{update U with equation~\ref{eqn::semi-mu-u}}
        \ENDWHILE
    \end{algorithmic}
\end{algorithm}

For the BCGD algorithm with semi-nonnegative $B$, we only change the update rule of
line 6 in Algorithm~\ref{alg::bcgd} to Equation~\ref{eqn::semi-b}.
\dingedit{Semi-nonnegative of the matrix B does not help from the experiment!}

\subsection{Model evolution with time}
Basically, we assume that the matrix $B$ should stay stable, 
while the matrix $U$ is evolving over time.

\subsubsection{Transition matrix}
The idea is to learn a transition matrix $A$ which approximates the changes of $U$ between
time $t-1$ to time $t$, i.e., $U_{t-1} = U_t A$, where $U \in R_+^{n\times k}, A \in R_+^{k \times k}$.

\noindent\textbf{Baseline.} One simple idea is to have a global transition matrix for the whole network. 
Therefore, the objective function with the baseline idea is as follows:
\begin{equation}
\label{eqn::baseline}
J_1=\sum_t\big(||G_t-U_tBU_t^T||_F^2 + ||U_t-U_{t-1}A||_F^2\big) + \lambda\sum_tTr(U_t^TLU_t)
\end{equation}

However, the transition of individual node might behave differently. 
Intuitively, if we have a local transition matrix $A_i$ for each 
individual node $i$, we should have better estimate accuracy. In that case,
the complexity of training transition matrix per node could be very high. Therefore,
to find a trade-off between model complexity and estimate accuracy, we propose the following
two ideas.

\dingedit{Depends on the performance, we should consider the possibility of using different 
    transition matrix at different timestamps.}

\subsubsection{Idea one: a two-step framework}
The idea is to first cluster the nodes into different parts based on their temporal behaviors,
then learn a transition matrix for each cluster.

We argue that the nodes with similar patterns behave similarly, i.e., with the same transition matrix.
Suppose we already have a clustering algorithm which groups the nodes into different clusters $C_i$,
then the objective function could be expressed as follows:

\begin{equation}
J=\sum_t\big(||G_t-U_tBU_t^T||_F^2 + \sum_{C_i}||U_t^{C_i}-U_{t-1}^{C_i}A^{C_i}||_F^2\big)
\end{equation}

To group the time series pattern, we could use any clustering algorithms for 
time series data~\cite{wang2006characteristic}. Alternately, we could also
use the idea of NMF with the following formulation:

\begin{equation*}
\arg\min_{W,H}||X-WH||_F^2
\end{equation*}

where $X \in R_+^{n\times t}$ is a matrix contains a time-series data for each node of the graph.
The idea is to decompose $X$ into two smaller matrices $W$ and $H$, where $W$ represents the weight
of each component in $H$. We cluster based on the matrix of $W$.

\dingedit{Idea one is too adhoc, abandoned.}

\subsubsection{Idea two: a unified framework}
In the two-step framework, we assume that the spatial and temporal properties are independent 
of each other. However, in the unified framework, we put the spatial and temporal attributes in 
one unified latent space, thus jointly infer both the spatial and temporal attributes together. 
Through this way, we only need one global transition matrix because it captures both the 
spatial and temporal evolutions. The objective function could be expressed as follows:

\begin{equation}
J_2=\sum_t\big(||G_t-U_tBU_t^T||_F^2 + ||X_t -U_tV||_F^2+ ||U_t-U_{t-1}A||_F^2\big)
\end{equation}

In this formulation, $X_t$ represents a node-feature matrix at each time stamp
which captures the temporal features of nodes, and we only learn one global
transition matrix $A$ for the whole nodes. 

\subsection{Algorithms of Solving Equation~\ref{eqn::baseline}}

\subsubsection{Multiplicative Update}
Take the derivative in respect of $U$, $A$ and $B$, we have the following:

\begin{small}
\begin{equation}
\begin{aligned}
    \frac{\partial J}{\partial U_\tau}=&-2(Y\odot G_\tau)(U_\tau B_\tau^T+U_\tau B_\tau) + 
    2(Y\odot U_\tau B_\tau U_\tau^T)(U_\tau B_\tau^T+U_\tau B_\tau)\\
    &+ 2(U_\tau-U_{\tau-1}A) + 2(U_{\tau}AA^T-U_{\tau+1}A^T) + 2\lambda LU_{\tau}\\   
\end{aligned}
\end{equation}
\end{small}

\begin{small}
\begin{equation}\label{eqn::temporal-aderi}
     \frac{\partial J}{\partial A}=-2\sum_{\tau=2}^{t}U_{\tau-1}^TU_\tau+2\sum_{\tau=2}^{t}U_{\tau-1}^TU_{\tau-1}A\\
     %\frac{\partial J}{\partial B}&=-2U^T(Y\odot G)U + 2U^T(Y\odot UBU^T)U
\end{equation}
\end{small}

\begin{small}
\begin{equation}\label{eqn::temporal-bderi}
\frac{\partial J}{\partial B}=-2\sum_{\tau=1}^{t}U_\tau^T(Y\odot G)U_\tau + 2\sum_{\tau=1}^{t}U_{\tau}^T(Y\odot U_{\tau}BU_{\tau}^T)U_{\tau}
\end{equation}
\end{small}

Because $B$ tends to be stable, the other way of choosing $B$ is to first aggregate all the graph snapshots and
find the average graph $G_{mean}$, we could factorize $B_{mean} = UB_{mean}U^T$ and use $B_{mean}$ as 
a fixed $B$ throughout Algorithm~\ref{alg::temporal-mu}.

\dingedit{How should we update B, assume that B should stay stable?}

\begin{algorithm}\small\caption{Temporal-MU}
    \textbf{Input:} graph matrix $G_1, G_2, \cdots, G_t$.\\
    \textbf{Output:}  $U_\tau$ ($1\leq \tau \leq t$), $A$ and $B$. \\
    \vspace{-2mm}
    \label{alg::temporal-mu}
    \begin{algorithmic}[1]
        \STATE{Initalize $U_{\tau}$ and $B$}
        \WHILE{Not Convergent}
            \FOR{$\tau = 1$ to $t$}
                \STATE{$U_{\tau}(ij)\leftarrow U_{\tau}(ij) \Big(\frac{[(Y\odot G)(U_{\tau}B_{\tau}^T+U_{\tau}B_{\tau})+U_{\tau-1}A+U_{\tau+1}A^T+\lambda WU_\tau]_{ij}}{[(Y\odot U_{\tau}B_{\tau}U_{\tau}^T)(U_{\tau}B_{\tau}^T+U_{\tau}B_{\tau})+U_{\tau}+U_{\tau}AA^T+\lambda DU_\tau]_{ij}}\Big)^\frac{1}{4}$}
                \STATE{$A({ij})\leftarrow A({ij}) \Big(\frac{[U_{\tau-1}^TU_{\tau}]_{ij}}{[U_{\tau-1}^TU_{\tau-1}A]_{ij}}\Big)$}
            \ENDFOR
            \STATE{$B_{ij}\leftarrow B_{ij} \Big(\frac{[\sum_{\tau=1}^{t}U_{\tau}^T(Y\odot G_{\tau}) U_{\tau}]_{ij}}{[\sum_{\tau=1}^{t}U_{\tau}^T(Y\odot (U_{\tau}BU_{\tau}^T))U_{\tau}]_{ij}}\Big)^\frac{1}{2}$}
        \ENDWHILE
    \end{algorithmic}
\end{algorithm}

\subsubsection{Block coordinate gradient descent}
We use the block coordinate gradient descent method, at one specific time $\tau$
between 1 to $t$:

\begin{equation}\label{eqn::temporal-uideri}
\begin{aligned}
&\Delta{J_{\tau}(u_i)} =
-2\sum_{j \in In(i)}\big(G_{\tau}(i,j)-u_{\tau}(i)Bu_{\tau}^T(j)\big)u_{\tau}(j)B^T\\
&-2\sum_{j \in Out(i)}\big(G_{\tau}(j,i)-u_{\tau}(j)Bu_{\tau}^T(i)\big)u_{\tau}(j)B + 2\big(u_{\tau}(i)-u_{\tau-1}(i)A\big)\\
&+2\big(u_{\tau}(i)AA^T-u_{\tau+1}(i)A^T\big)
\end{aligned}
\end{equation}

\begin{algorithm}\small\caption{Temporal-BCGD}
    \textbf{Input:} graph matrix $G_1, G_2, \cdots, G_t$.\\
    \textbf{Output:}  $U_\tau$ ($1\leq \tau \leq t$), $A$ and $B$. \\
    \vspace{-2mm}
    \label{alg::temporal-bcgd}
    \begin{algorithmic}[1]
        \STATE{Initilize $U_{\tau}$ and $B$}
        \WHILE{Not Convergent}
            \FOR{$\tau = 1$ to $t$}
                \FOR{each $i \in G$}
                    \STATE{$u_{\tau}(i) \leftarrow \max\big(u_{\tau}(i) - \alpha \Delta{J(u_{\tau}(i))}, 0\big)$ with Equation~\ref{eqn::temporal-uideri}}
                \ENDFOR
                \STATE{$ A \leftarrow \max(A - \alpha \frac{\partial J}{\partial A}, 0)$ with Equation~\ref{eqn::temporal-aderi}}
            \ENDFOR
            \STATE{$ B \leftarrow \max(B - \alpha \frac{\partial J}{\partial B}, 0)$ with Equation~\ref{eqn::temporal-bderi}}
        \ENDWHILE
    \end{algorithmic}
\end{algorithm}

%\begin{equation}
%\begin{aligned}
%\Delta_{J_1}(A) = -U_{\tau-1}^TU_\tau-U_\tau^TU_{\tau-1}+2AU_{\tau-1}^TU_{\tau-1}
%\end{aligned}
%\end{equation}
%
%\begin{equation}
%\begin{aligned}
%\Delta_{J_1}(B) = -2U_{\tau}^TU_{\tau}(G-U_{\tau}BU^T_{\tau})
%\end{aligned}
%\end{equation}

\subsection{Confidence Level Computation}

\subsection{Incremental Update}
At time $t+1$, once we received the true readings, we need to adjust the latent space.
The basic algorithm is shown in Algorithm~\ref{alg::incremental-update}, we maintain a 
candidate set and only adjust the latent space of the nodes in the candidate set.

\begin{algorithm}\small\caption{Incremental-Update($U_{t+1}, \widehat{G_{t+1}}, G_{t+1}$)}
    \textbf{Input:}  $U_{t+1}$, predicted graph reading $\widehat{G_{t+1}}$, observed graph reading $G_{t+1}$.\\
    \textbf{Output:}  Updated latent space $U_{t+1}$. \\
    \vspace{-2mm}
    \label{alg::incremental-update}
    \begin{algorithmic}[1]
        \STATE{$cand \leftarrow \emptyset$}
        \FOR{each $i \in G$}
            \FOR{each $j \in out(i)$}
            \IF{$|G(i,j) -\widehat{G(i,j)}| \ge \delta $}
                \STATE{$cand \leftarrow cand \cup \{i,j\}$}
            \ENDIF
            \ENDFOR
        \ENDFOR
        \WHILE{Not Convergent AND $cand \notin \emptyset$}
             \FOR{each $i \in G$}
                 \STATE{update $u_{t+1}(i)$ with MU or BCGD}
             \ENDFOR
             \FOR{each $i \in cand$}
                \IF{$norm(u_{t+1}(i))-norm(u_{t+1}(i)_{old}) \leq \Delta$}
                    \STATE{$cand \leftarrow cand \setminus \{i\}$}
                \ENDIF
                \FOR{each $j \in out(i)$}
                    \STATE{$p \leftarrow u_{t+1}(i)Bu_{t+1}(j)$}
                    \IF{$|p-{G(i,j)}|\geq \lambda $}
                        \STATE{$cand \leftarrow cand \cup \{j\}$}
                    \ENDIF
                \ENDFOR
             \ENDFOR             
        \ENDWHILE
    \end{algorithmic}
\end{algorithm}

On the other hand, we could adjust the latent space of one node to its correct position at one time, then adjust the other influenced nodes correspondingly. In this way, we need to find a new $u(i)$ such that the updated $u(i)$ could produce the correct result, 
assume that we already have $u_t(i), u_t(j)$ and $B$.

\begin{equation}
\begin{aligned}
    u_{t+1}(i) &=\arg\min_{u(i)}\frac{1}{2}||u(i)-u_{t}(i)||_F^2 \\
    \mbox{s.t.} \quad &|u(i)Bu^T_t(j)-G(i,j)| \leq \delta
\end{aligned}
\end{equation}

We have a closed form solution for the optimization problem:

\begin{equation}
\begin{aligned}
u_{t+1}(i) &= u_t(i) + sign(\widehat{G(i,j)}-G(i,j)) \cdot \frac{\widehat{G(i,j)}-G(i,j)-\delta}{||x_t||^2}x_t\\
\mbox{where \quad} &x_t = (Bu^T_t(j))^T = u_t(j)B^T
\end{aligned}
\end{equation}


==> tex/relate.tex <==
% related work
